ParaBank: Monolingual Bitext Generation and Sentential Paraphrasing via Lexically-constrained Neural Machine Translation

We present ParaBank, a large-scale English paraphrase dataset that surpasses prior work in both quantity and quality. Following the approach of ParaNMT, we train a Czech-English neural machine translation (NMT) system to generate novel paraphrases of English reference sentences. By adding lexical constraints to the NMT decoding procedure, however, we are able to produce multiple high-quality sentential paraphrases per source sentence, yielding an English paraphrase resource with more than 4 billion generated tokens and exhibiting greater lexical diversity. Using human judgments, we also demonstrate that ParaBank's paraphrases improve over ParaNMT on both semantic similarity and fluency. Finally, we use ParaBank to train a monolingual NMT model with the same support for lexically-constrained decoding for sentence rewriting tasks.

==> bleuall.tex <==
\begin{table*}[tbp]
\centering
\begin{tabular}{cl|lllll|lllll}
\toprule
     \# &     System  & \multicolumn{5}{c}{Czech-English} & \multicolumn{5}{c}{French-English} \\
         &             &  len=5 &  len=10 &  len=20 &  len=40 &  Overall &len=5 &  len=10 &  len=20 &  len=40 &  Overall \\
\midrule
35 & \textsc{ParaNMT} &     18.32 &   25.49 &   32.25 &   33.84 &    27.48 &        - &         - &         - &         - &          - \\
17 &  $\ominus$3rd low IDF &  \bf{9.25} &\bf{20.62}&   35.76 &   41.88 &\bf{26.88}&     6.59 &     15.57 &     26.78 &     34.54 &      20.87 \\
21 &    $\ominus$3 low IDF & \bf{0.00}  &\bf{7.84}&\bf{22.04}&\bf{28.90}&\bf{14.70}&     1.21 &      6.90 &     18.28 &     22.02 &      12.10 \\
28 &         no con. &  19.32     &   28.41 &   42.02 &   46.63 &    34.10 &    14.07 &     21.12 &     30.57 &     38.66 &      26.11 \\
31 &  $\oplus$3rd top IDF &  19.09     &   29.16 &   41.42 &   46.96 &    34.16 &    15.28 &     21.69 &     31.49 &     37.56 &      26.51 \\
34 &  $\ominus$first 3 tks & \bf{13.22} &\bf{24.90}&   39.11 &   44.67 &    30.47 &    10.87 &     18.15 &     27.70 &     36.87 &      23.40 \\
\midrule
35 &        PPDB equ &      - &       - &       - &       - &        - &     4.46 &     13.33 &     25.88 &     29.54 &      18.30 \\
36 &        PPDB fwd &      - &       - &       - &       - &        - &     1.51 &      8.87 &     14.14 &     19.03 &      10.89 \\
37 &        PPDB bkw &      - &       - &       - &       - &        - &     3.94 &      9.69 &     18.94 &     26.24 &      14.70 \\
\bottomrule
\end{tabular}
\caption{Modified BLEU scores computed between concatenated paraphrases and concatenated reference sentences of length 5, 10, 20, and 40. \textbf{Lower} BLEU score suggests higher lexical diversity. Because each plot orders systems left to right by increasing semantic similarity scores (\tabref{tab:MTurk_score}), any system that is to the right of ParaNMT with a lower BLEU score demonstrates both greater lexical diversity \textit{and} semantic similarity.}
\label{tab:BLEU_score}
\end{table*}

%

%
%
%
%

==> humanjudged.tex <==
\begin{table*}[tbp]
\centering
\begin{tabular}{cl|lllll|lllll}
\toprule
     \# &     System  & \multicolumn{5}{c}{Czech-English} & \multicolumn{5}{c}{French-English} \\
         &             &  len=5 &  len=10 &  len=20 &  len=40 &  Overall &len=5 &  len=10 &  len=20 &  len=40 &  Overall \\
\midrule
   - &         \textsc{ParaNMT} &   73.47      & 73.49      &    75.49      & 71.09      & 73.39       &-&-&-&-&- \\
   17 &  $\ominus$\trd low IDF &   71.59      & \bf{75.71} &    \bf{79.67} & \bf{77.31} & \bf{76.07} &73.64 &               72.69 &               83.60 &               80.15 &    77.52  \\
   21 &    $\ominus$3 low IDF &   59.86      & 66.56      &    70.76      & 69.77      & 66.74      &62.84 &               69.56 &               81.73 &               77.08 &    72.80  \\
   28 &         no con. &   \bf{76.63} & \bf{78.35}* &    \bf{83.19}* & \bf{80.35} & \bf{79.63}* &79.09 &               74.28 &               84.86 &               83.02* &    80.31*  \\
   31 &  $\oplus$\trd top IDF &   \bf{77.12}* & \bf{75.22} &    \bf{82.98} & \bf{79.91} & \bf{78.81} &80.22* &               73.78 &               85.01 &               80.02 &    79.76  \\
   34 &  $\ominus$first 3 tks &   \bf{74.03} & \bf{77.74} &    \bf{81.88} & \bf{81.04}* & \bf{78.67} &78.12 &               74.37* &               84.14 &               82.74 &    79.84 \\
\midrule
35 &        PPDB Equ &  -&-&-&-&-&           79.22 &               67.30 &               82.09 &               79.98 &    77.15 \\
  36 &        PPDB Fwd &   -&-&-&-&-&           65.40 &               69.39 &               85.10* &               82.75 &    75.66 \\
  37 &        PPDB Rev &   -&-&-&-&-&           64.25 &               66.28 &               76.35 &               72.49 &    69.84 \\
\bottomrule
\end{tabular}
\caption{Semantic similarity between paraphrase and reference sentences, as scored by human annotators on a 0-100 scale (least to most similar). Results are grouped by length of reference sentence \{5, 10, 20, 40\}.
%
%
%
System names and numbers correspond to \tabref{tab:system_description}.
%
Improvements over \textsc{ParaNMT} for Czech-English in bold. Asterisk (*) indicates best in column.}
\label{tab:MTurk_score}
\end{table*}
